Research on access, use and effective exploration of astronomical observational and bibliographical data from sonification

Data analysis in space sciences has been performed exclusively visually for years, despite the fact that the largest amount of data belongs to non-visible portions of the electromagnetic spectrum. This, on the one hand, limits the study of the unknown to the current resolution possibilities of the screens, and on the other hand, it excludes a group of people who present some type of visual disability. Taking into account the aforementioned, and that people with some type of disability encounter many barriers to achieve academic studies and stable jobs, the present investigation focuses on new modalities of access to the data, but taking into account the accessibility and inclusion of people with functional diversity from the beginning. It has been shown that multimodal perception (use of more than one sense) can be a good complement to visual exploration and understanding of complex scientific data. This is especially true for astrophysical data, composed of a sum of different oscillatory modes resulting in the final complex data array. This proposal focuses on the human ability to adapt to data and interaction with sound, in order to analyze data sets and produce an application aimed at leveling the possibilities of access to information in the field of physics and astronomy (although the tool is also applicable to any type of data in files with 2 or more columns (.txt or .csv)) for people with disabilities. In addition, it proposes the study of scientific and technological capacities for the generation of tools with a novel approach, focused on the user and oriented to: a specific social problem, the use of free programming languages and the design of infrastructure to improve inclusion.

==> chapters/capitulo_actividades.tex <==

Con base en lo descripto hasta el momento, se definieron las acciones a seguir para poder llevar adelante los objetivos de esta disertación: \textit{``Investigar sobre nuevas modalidades de acceso a los datos astronómicos y astrofísicos, promoviendo la inclusión en los espacios científicos y buscando mejorar la forma de despliegue actual''} y \textit{``Producir herramientas y documentación orientada a mejorar el acceso a los datos promoviendo la inclusión''}. Lo descripto en cada uno de los párrafos siguientes será detallado en capítulos particulares de la versión final del manuscrito de esta tesis.

Como actividad inmediata, posterior a los resultados obtenidos de la investigación presentada en el Capítulo \ref{cap:analisis_normativo}, se estableció el desarrollo de la primer versión de SonoUno. Dicho desarrollo se comenzó desde cero, en lenguaje Python, utilizando el entorno de desarrollo Spyder y un repositorio online publicado en GitHub. Todas estas herramientas se mantienen hasta la actualidad, habiendose logrado un software de sonorización de datos, programado completamente en Python, de acceso libre y con evidencias de uso en diferentes partes del mundo (se ha tenido contacto con el `Centro de Astrofísica y Supercomputación, de la Universidad de Swinburne (Swinburne University of Technology), Australia', el `Observatorio Astrofísico Smithsoniano (Smithsonian Astrophysical Observatory), Cambridge, Estados Unidos' y `Carlos Morales Socorro, Asesor educativo en el CEP Las Palmas, Universidad de Las Palmas de Gran Canaria', entre otros). 

Una vez que se obtuvo la primer versión del programa de sonorización, a principios del año 2019, se realizó un estudio con Grupo Focal para evaluar la accesibilidad y usabilidad del mismo. El estudio decantó en buenos resultados y nuevas propuestas y modificaciones para mejorar la accesibilidad de sonoUno. El proceso y los resultados fueron publicados a inicios de 2022 en una revista \citep{casadoFG2022}. Un resumen más detallado de esta actividad se ofrece en la sección \ref{sect:act_realizadas}.

Como se mencionó anteriormente, se utiliza la plataforma GitHub como repositorio del código fuente del programa (la primera publicación se realizó en mayo de 2019 y la última actualización a principios de junio de 2022, \url{https://github.com/sonoUnoTeam/sonoUno/}). Las actualizaciones que van surgiendo como resultado de cada investigación, se suben en dicho repositorio utilizando diferentes ramas paralelas a la rama principal, para mantener en la rama principal solo la última versión estable. Además, el uso del repositorio y las diferentes ramas nos permite que todos los desarrolladores que deseen aportar al programa puedan hacerlo de una forma ordenada y con registro de todos los cambios que se realizan al mismo.

Dado que el programa ha sido de interés para diferentes institutos de investigación y divulgación de la ciencia, para poder agilizar y mejorar la comunicación y transmisión de la información, se crea una página web dedicada al proyecto. En dicha web (que se crea siguiendo las recomendaciones y lineamientos descriptos en el Capítulo \ref{cap:analisis_normativo}) se encuentran información general, el archivo con las recomendaciones de accesibilidad, los manuales, instructivos de instalación, el acceso a la versión web, el acceso a github y una galería donde se presentan diferentes datos astronómicos ingresados al programa (\url{https://www.sonouno.org.ar}).

Las actualizaciones periódicas del software, respondiendo a los comentarios de los usuarios, han sido realizadas durante todo el proceso de esta tesis. La finalidad es alcanzar una herramienta que sea útil, usable, eficaz y eficiente para la investigación en astronomía por personas con diversidad funcional; al mismo tiempo que los intercambios con usuarios nos permiten ampliar la investigación propia. Siendo más específicos, en base a cada intercambio con usuarios, se diseñan las actualizaciones de acuerdo con los comentarios recibidos y así se pautan las tareas a realizar antes de volver a enviar el programa a usuarios para ser nuevamente probado; registrando todo el intercambio para poder comparar las necesidades de los diferentes grupos y evaluar características que permitan elaborar bases que apoyen o modifiquen el marco de trabajo propuesto.

Durante el desarrollo de esta tesis, se participó en el proyecto REINFORCE (REsearch INfrastructures FOR Citizens in Europe) (\url{www.reinforceeu.eu}) (diciembre, 2019 - actualidad). Mediante dicha participación se buscó potenciar el desarrollo del software. En el caso particular de este proyecto se busca usar el SonoUno para sonorizar ondas gravitacionales, fuentes marinas de ruido en el detector KM3NeT, partículas en el Gran Colisionador de Hadrones e imágenes de muones. Durante este último tiempo se trabajó para el acceso y sonorización de archivos con grandes cantidades de datos, hasta el momento se ha probado ingresar archivos de dos columnas y hasta un millón de filas. Se realizó un script para poder generar archivos de sonido en bash utilizando las librerías de sonoUno. Se produjo un script y la posterior integración al software, para la sonorización de datos de partículas en el Gran Colisionador de Hadrones. Adicionalmente, se logró una primer versión de sonorización de imágenes y de datos de muones.

En cuanto a las publicaciones y la transferencia, se lograron dos publicaciones en revista este año \citep{casadoFG2022,casadoiso2022} (la publicación referente a la normativa es la descripta en el Capítulo \ref{cap:analisis_normativo}; en cuanto a la publicación que describe el análisis con grupo focal, se adjunta en el Apéndice \ref{ap:FG}). Además, se han realizado diferentes publicaciones en congreso y se han recibido diferentes invitaciones a congresos, las más relevante a esta disertación son las invitaciones al Audible Universe Workshop. La primer invitación a dicho evento fue en agosto de 2021, durante el evento el equipo de trabajo se reunioó con referentes de sonorización multidisciplinares para discutir sobre las bases de la sonorización y posibles pasos a seguir. Producto de dicho encuentro se escribió un artículo científico presentado en la revista `Nature', donde \citet{zanella2022} describen el estado actual de los programas de sonorización y un repositorio que se hizo posterior al encuentro. En dicho trabajo presentan al desarrollo sonoUno como uno de los software que tiene a la accesibilidad como objetivo principal (solo el 13\% de los desarrollos incluidos lo comparten) y al público en general e \textbf{investigadores} como usuarios principales (no llegan al 50\% los software que apuntan a investigadores como usuarios). Este reconocimiento a nivel internacional se considera muy beneficioso para la presente tesis y sus proyecciones futuras. Se desea agregar que se organizó un segundo evento que tendrá lugar a fin de este año, al cual también fue invitado el equipo de trabajo y ya se confirmó asistencia.

\section{Descripción de la investigación realizada con Grupo Focal}
\label{sect:act_realizadas}

A principios de 2019 se realizó un trabajo en conjunto con la Universidad de Southampton para llevar a cabo un grupo focal con potenciales usuarios del SonoUno. En dicho marco se llevaron a cabo los grupos focales, donde se buscaba probar si el software y su interfaz de usuario es usable, efectivo y eficiente.
Durante las pruebas se detectaron errores en el programa que fueron corregidos luego de las pruebas. También se evidenciaron problemas de accesibilidad y diferentes funcionalidades necesarias, de los cuales algunos han podido ser incluidos y otros continúan pendientes. Dichos hallazgos y actualizaciones fueron publicadas en un proceeding publicado a partir de una charla en el congreso de la IAUS 367 en el año 2020, además, se está escribiendo un paper dedicado al desarrollo del software donde se incluyen las actualizaciones realizadas este último año.

En cuanto a los resultados del grupo focal propiamente dicho el paper ya está escrito y se está enviando a revista. En el mismo se detalla el proceso de análisis de las transcripciones obtenidas, que fue realizado por dos personas utilizando la técnica de condensación de texto \citep{malterud2012} y un análisis de confiabilidad posterior. El resultado del análisis de confiabilidad dió un valor aceptable que permite decir que los resultados son confiables. Se definieron en el proceso cinco categorías que engloban las afirmaciones más relevantes hechas por los participantes:
\begin{itemize}
    \item Sobrecarga de memoria: hace referencia a la carga cognitiva que requiere la realización de una tarea determinada, esta categoría incluye comentarios donde la carga cognitiva producida por el uso del programa es mucha, como así también cuando el software favorece la carga cognitiva.
    \item Necesidad de información: agrupa la necesidad de que el programa de información sobre determinadas tareas, sobre todo cuando se usa con lector de pantalla, y también, la necesidad de información sobre el programa en sí mismo y las tareas que permite realizar.
    \item Necesidad de poder elegir: las afirmaciones que incluye esta categoría no solo remarcan la necesidad de poder elegir frente a diferentes opciones, sino también que el programa en desarrollo les permitió poder tomar decisiones sobre cómo querían trabajar con los datos, cosa que actualmente no es posible para personas con diversidad funcional.
    \item Necesidad de entrenamiento: esta categoría se define en base a que se evidencia falta de conocimiento en el uso de sonido para analizar los datos, y en paralelo la necesidad de entrenamiento con el uso mismo del programa en desarrollo.
    \item Aspectos sociales: parte de las afirmaciones realizadas por los participantes ponen en evidencia por un lado como en general los desarrolladores no tienen en cuenta las diversidades funcionales y la inclusión. Por otro lado, se evidencia la falta de entendimiento por parte de las personas sin discapacidad, ya que ese grupo de personas expresó no creer que las personas con discapacidad pudieran hacer ciencia.
\end{itemize}

Se concluye y refuerza en este trabajo, la necesidad de una herramienta que ofrezca autonomía a las personas con discapacidad y permita su inclusión en el campo de trabajo donde se desarrollen. Esto último hace referencia a la necesidad de herramientas que se adapten a las necesidades del usuario, permitiendo ser usadas por personas con y sin discapacidad, obteniendo los mismos resultados. Se remarca la importancia de incluir a los usuarios finales desde el inicio, este trabajo dio lugar a reajustar funcionalidades que no eran útiles como se esperaba; por ejemplo, se esperaba que una barra deslizable para ajustar el límite inferior y superior de la gráfica fuera más fácil de usar con el teclado, que el ingreso de números específicos en un espacio de texto, pero tanto usuarios discapacitados como sin discapacidad prefieren un espacio para indicar el número específico ya que eso permite precisión.

Se resalta en este trabajo por parte de las personas con discapacidad visual que la herramienta les da la posibilidad de ser autónomos y realizar tareas que en la actualidad no les es posible. En base a esto se cree que una herramienta usable por personas con diversidad funcional es posible a largo plazo, sobre todo con un enfoque modular que permite ir agregando funcionalidades a medida que se realizan los estudios y pruebas pertinentes.


==> chapters/conclusion_ant.tex <==

A partir del inicio de esta tesis doctoral en 2017, se ha evidenciado un crecimiento exponencial de programas y técnicas de sonorización de datos astronómicos y astrofísicos (entre otros), marcando el pulso de estos tiempos en que la aproximación multimodal al estudio de la naturaleza se perfila como tema de alto impacto en el ámbito científico. Sin embargo, el enfoque de la investigación realizada y el permanente compromiso con la inclusión y el diseño centrado en el usuario, ha posibilitado que sonoUno logre diferenciarse de sus pares y que el equipo de trabajo sea reconocido en el ámbito científico internacional como un referente \citep{zanella2022}.

Respecto de las técnicas de sonorización, si bien existen algunos antecedentes antes de los '90, la mayoría de los desarrollos y publicaciones que evidencian su uso en ciencia y divulgación son posteriores. De acuerdo a \citet{zanella2022}, los últimos cinco años igualó en porcentaje de desarrollos nuevos, a los 20 años previos. Esto muestra la necesidad que existe por parte de los científicos, de nuevas técnicas de despliegue de datos, reforzando la premisa de que un despliegue multimodal permite un mejor análisis de los mismos.

Teniendo en cuenta que un despliegue multimodal, además, permite el acceso a los datos para personas con diferentes estilos sensoriales (por ejemplo, personas ciegas, a las cuales el actual despliegue de datos deja excluidas), es que se complementa en esta tesis la investigación de nuevas técnicas de visualización con el desarrollo de herramientas centradas en el usuario y accesibles desde el inicio. De esta forma se logró una herramienta que no solo mejora el actual despliego de los datos, sino que además, permite la inclusión de personas con diversidad funcional en el ámbito científico.

En cuanto a los objetivos planteados inicialmente:

\begin{itemize}
	\item Investigar sobre nuevas modalidades de acceso a los datos astronómicos y astrofísicos, promoviendo la inclusión en los espacios científicos y buscando mejorar la forma de despliegue actual;
	\item Producir herramientas y documentación orientada a mejorar el acceso a los datos promoviendo la inclusión;
\end{itemize}

Se logró desarrollar nuevas modalidades de acceso a los datos (mediante la sonorización), pudiendo mostrar el despliegue gráfico de la misma forma que se muestra en otros programas o bases de datos, siendo acompañado por la sonorización de dichos datos. Se debe tener en cuenta que todas las sonorizaciones producidas en el marco de esta tesis doctoral representan fielmente los datos, no se les aplica ningún tipo de "maquillaje'' para que suene bonito, lo que permitió mantener claro que es un desarrollo que busca insertarse en el ámbito científico. Las sonorizaciones de tablas de dos o más columnas se basaron en las sonorizaciones realizadas por el software xSonify. No obstante, las sonorizaciones de partículas fue diseñada desde cero como parte de esta tesis.

Las investigaciones realizadas con usuarios y otros grupos de investigación, sobre el uso y la accesibilidad del software sonoUno para el análisis de datos, han sido favorables, demostrando que el programa presenta un marco de trabajo centrado en el usuario y en la inclusión. En base a estos intercambios también se han podido producir guías de trabajo y documentación sobre recomendaciones de accesibilidad que se encuentran disponibles en la \href{https://www.sonouno.org.ar/}{\underline{\textcolor{blue}{web de sonoUno}}} (sección \ref{sect:recomendaciones_publicadas}). Todas estas actividades han sido acompañadas por análisis de normativas vigentes para mantener un marco de trabajo lo más completo y actualizado posible.

En base a los continuos intercambios con usuarios, se materializó la necesidad de que el desarrollo fuera más allá de una simple interfaz gráfica de escritorio. Así se comenzó con el desarrollo de una interfaz gráfica web que alcanzó un alto nivel de funcionalidades, igualando y mejorando en algunos aspectos al inicial desarrollo de escritorio. El proyecto sonoUno y en particular la investigación de esta tesis, logró mantener y llevar a cabo sus objetivos iniciales, promoviendo la inclusión en el ámbito científico y convirtiéndose en un referente de sonorización para el análisis multisensorial de datos. 

Si bien sonoUno cuenta con varios casos de uso donde se trabaja la divulgación en el ámbito científico y la educación (ver sección \ref{sect:casos_uso}, adicionalmente se puede ver el uso de sonoUno en Raspberry Py implementado por \href{https://github.com/Physicslibrary/SonoUno-Raspberry-Pi}{\underline{\textcolor{blue}{Hartwell Fong}}}), sigue siendo un desarrollo enmarcado en el ámbito científico. Desde el inicio se ha trabajado con datos reales, descargados desde grandes bases de datos (ver sección \ref{sect:cap6_vescritorio}) o proporcionados por grandes facilidades astrofísicas (ver sección \ref{sect:cap6_sonif_reinforce}). De las encuestas realizadas en los últimos años, la mayoría de los científicos que han utilizado el software estaría dispuesto a utilizarlo en sus investigaciones, siempre que el programa se mantenga en desarrollo y continúe mejorando. En base a esta última premisa, resaltó la necesidad de entrenamiento sobre esta nueva modalidad de despliegue multisensorial de datos.

Es así que la línea de investigación que se presenta en este trabajo, deja establecida la posibilidad de mejora continua del software (ver sección \ref{sect:cap7_lineastrabajo}) pero, además sienta las bases para numerosos trabajos futuros en diferentes líneas de investigación: 

\begin{itemize}
	\item Análisis de percepción: durante el curso internacional de entrenamiento realizado en el marco de la escuela de verano 2022 del proyecto REINFORCE (ver sección \ref{sect:cap7_workshopjul2022}), se realizó una encuesta donde se evidenció la necesidad de entrenamientos, entre otras cosas. Si bien dicho evento se enfocó mayormente en las sonorizaciones de nuevos datos como las partículas del LHC, la necesidad de entrenamiento no se limita a los nuevos diseños de sonorizaciones. Se ha evidenciado durante todo el desarrollo de esta tesis y a lo largo de diferentes encuestas, la necesidad de entrenamiento tanto en el uso de la técnica de sonorización, como en el uso de la herramienta sonoUno. Incluso durante el último workshop de sonorización (\textit{``The Audible Universe 2''}) se discutió sobre la necesidad de entrenamientos para instruir a las personas en el uso del despliegue multisensorial de datos. Es importante destacar que relacionado a este tema, se ha presentado en la Carrera de Bioingeniería de esta Universidad un trabajo final de grado titulado \textit{``Desarrollo de entrenamientos para el análisis multisensorial de datos''}, donde se describen los primeros pasos con el desarrollo y puesta en marcha de entrenamientos, y la elaboración de una web propia para el despliegue de dichos entrenamientos. Adicionalmente, la misma estudiante dentro de el grupo de investigación donde se desarrolló esta tesis, comenzaría este año su tesis doctoral con beca CONICET (ya otorgada para comenzar en abril de 2023) titulada \textit{``Investigación interdisciplinaria de la efectividad de los entrenamientos en sonorización de datos astronómicos en el marco de la astrofísica multimodal''}.
	
	\item Nuevas técnicas de diseño centrado en el usuario: entre ellas se puede mencionar las interfaces que se adapten al usuario, que aprendan de la interacción con el mismo e inteligencia artificial, entre otras. Si bien se encuentran numerosos esfuerzos por alcanzar interfaces centradas en el usuario y que promuevan la inclusión, pocos de ellos se mantienen a largo plazo, ya sea por falta de fondos o por la dificultad de encontrar una técnica que se acomode a todos. Adicionalmente, si bien existen estándares que describen buenas prácticas para abordad la accesibilidad, no se logra evidenciar un consenso sobre la mejor forma de desplegar interfaces hombre computador que cumplan con los criterios de inclusión y sean atractivas para la mayoría de los usuarios.
	
	\item Nuevas técnicas de sonorización: si bien se ha avanzado mucho en materia de sonorización, falta mucho para lograr dar respuesta a los numerosos estilos de visualización de datos presentes en la actualidad (por ejemplo, sonorización de imágenes). Esto, sin perder de vista que lo que se busca es dar sentido a los datos a través de la sonorización: no es sonorizar un despliegue visual, sino representar un conjunto de datos a través de sonorización para poder analizarlos utilizando las diferentes entradas sensoriales del organismo humano (por ejemplo, no se utilizaría la misma técnica de sonorización para representar la imagen de una galaxia que la de un Glitch, eso es debido a que son conceptos diferentes e incluso su representación gráfica se origina de forma diferente).
	
	\item Tecnologías asistivas: durante el desarrollo de esta tesis se tuvieron en cuenta los lectores de pantalla de acceso libre y gratuito de cada sistema operativo, pero no son las únicas tecnologías asistivas disponibles. Dentro de este marco, se deberían incluir todas las tecnologías asistivas disponibles analizando la factibilidad de su uso con la herramienta sonoUno, como sería el caso de Alexa, teclados accesibles (cambia su diseño de acuerdo a la necesidad), tableros de comunicación, reconocimiento de voz, por mencionar algunas. Sin duda este trabajo excede los límites de esta tesis y es por ello que representa una de las líneas de trabajo a futuro que se desprende de esta tesis.
\end{itemize}

Las posibilidades de contribución en las mencionadas lineas de investigación constituyen un legado de alto impacto en el marco de una sociedad que pugna por la equidad, la inclusión y la sostenibilidad de estos principios. En base a las recomendaciones de la Naciones Unidas y basándonos en el \textit{``Estudio Nacional sobre el Perfil de las Personas con Discapacidad''} es evidente que se necesita tomar acción a largo plazo para asegurar la equidad, las diversidades funcionales que presentan las personas no deben ser un limitante para su desarrollo profesional. Los objetivos globales de equidad e inclusión requieren de marcos de referencia que emergen de estudios formales, que puedan ser utilizados como facilitadores para la remoción de las barreras que impiden el crecimiento y progreso social.


==> chapters/introduccion_ant.tex <==

Al iniciar la presente investigación y comenzar a utilizar la palabra `accesible', la cual derivada de la palabra accesibilidad, siempre se la relacionó con la habilidad de producir algo que pudiera ser utilizado por personas con diferentes capacidades sin que significara mayor dificultad para una u otra. Sin embargo, rápidamente, al tener relación con personas discapacitadas y comenzar a profundizar en el tema, la definición de accesibilidad fue cambiando.

Observando el término `discapacidad' y `accesibilidad' durante los últimos 50 años, la investigación sobre accesibilidad dejó de centrarse en la discapacidad como un problema médico o deficiencia que debía repararse, dando un giro hacia un constructo más social \citep{macketal2021}. Así, se comenzó a diferenciar entre la discapacidad como una condición física o biológica y la discapacidad como construcción social y ambiental. En el caso de esta tesis, el texto estará centrado en esta última definición de discapacidad, teniendo en cuenta todas las capacidades que tiene una persona y buscando reducir al mínimo las limitaciones que podría llegar a experimentar, principalmente en el caso de una interfaz humano-computadora. En este sentido es interesante pensar, además, en las dificultades a las que también se enfrentan las personas que se define (o autodefinen) como no discapacitadas, para abordar los desafíos que se detallan en del presente trabajo. Otro término que se utilizará ampliamente es `inclusión' que hace referencia a la necesidad de que el sistema, herramienta o entorno que se está desarrollando se ajuste a las necesidades o capacidades de todas las personas. Se debe tener en cuenta que este trabajo no busca investigar nuevas modalidades de acceso a los datos para personas con discapacidad, sino que busca investigar sobre estas nuevas modalidades promoviendo la inclusión en los espacios científicos y buscando mejorar el despliegue actual de los datos en astronomía y astrofísica.

En cuanto a la realidad laboral de las personas con discapacidad en Argentina, existen diferentes normativas que buscan reglamentar y promover la inclusión como ser: la ``Ley 22.431 - Sistema de protección integral de los discapacitados'', la Ley que reglamenta el certificado único de discapacidad, la ley que reglamenta el trasporte público adaptado e incluso la Ley 26.378 que aprueba la ``Convención sobre los Derechos de las Personas con Discapacidad y su protocolo facultativo'' elaborado y publicado por las Naciones Unidas. Sin embargo, datos del \citet{indec2018} muestran una realidad preocupante, solo un 32\% de las personas mayores a 14 años que sufren una o más discapacidades tienen un empleo. Otro inconveniente con el que se encuentran las personas con discapacidad es el acceso a la educación, un 20\% de las personas con discapacidad de 15 años o más han dejado sus estudios con un primario incompleto. De los que lograron terminar la primaria un 46\% no logró finalizar la secundaria, un 20\% logró terminarla y solo un 13\% accedió a algún tipo de educación superior. Se considera que tanto para el ámbito académico como laboral uno de los problemas fundamentales es la falta de herramientas y modalidades de presentación de la información que promuevan y generen inclusión.

Una realidad que llamó la atención, es que las prácticas de intercambio de información en todos los aspectos de las ciencias STEM, incluida la preparación académica y especialmente en matemáticas en la educación superior y las ciencias en las aulas escolares, pueden impedir que la mayoría de las personas participen, por ejemplo en el campo de la astronomía. Durante los últimos 100 años, la humanidad ha sido testigo de un cambio de mentalidad general hacia la naturalización del derecho humano inherente a la participación equitativa e igualitaria en las líneas actuales de investigación científica, como así también en educación y difusión de las ciencias.

Una extensa y profunda búsqueda bibliográfica sugirió que la falta de experimentos de percepción (aplicados al análisis de datos astronómicos), la brecha de desarrollo causada por los enfoques del conocimiento en cada momento de la historia de la ciencia y de la humanidad, el desempeño y los estilos de producción en el mercado laboral a medida que las máquinas se integraron en la investigación, acompañado por el desarrollo detenido de las tecnologías de audio (en comparación con las tecnologías visuales) y su aplicación a los factores humanos, contribuyeron a una disminución de las formas asociadas con otros tipos de experiencia sensorial y al predominio de formas uniformes de transmitir y analizar la información científica en general y astronómica en especial. En ese sentido, \citet{wandatesis2013} y \citet{mercedetal2011} investigaron si las modalidades visuales eran mejores que otras modalidades sensoriales para la exploración de datos astrofísicos a través de experimentos de percepción y encontraron que el uso del sonido aumentaba la sensibilidad del astrónomo experto frente a eventos en los datos que por naturaleza son: de muy baja relación señal/ruido; o bien, ambiguos para el ojo humano. 

Volviendo un poco a través de la historia, no hay evidencia experimental (para información astronómica) que respalde por qué la astronomía profesional dejó de usar otras modalidades sensoriales para el despliegue de datos bajo análisis, máximo si se tiene en cuenta que la mayor parte del espectro electromagnético (su principal objeto de estudio) se encuentra fuera del rango visible de longitudes de onda. Esto lleva a la pregunta de por qué la física y la astronomía han seguido utilizando las mismas transacciones e interacciones uniformes, digitales, cognitivas, expresivas y reflexivas. Esto puede deberse a la falta de evidencia experimental, a la curva de aprendizaje, al lento progreso de la resolución de audio o los métodos de aprendizaje uniformes (educación superior), entre otros. Sin embargo, ciertamente está claro ahora que la mayoría de las personas videntes usan sus ojos para dar sentido a su mundo, y esta es la modalidad sensorial humana predominante, que se utiliza para dar sentido consciente al conocimiento astronómico.

La presente disertación expone la investigación realizada sobre el uso del despliegue multimodal (a través de sonido como anexo a la visualización) de datos para evaluar la accesibilidad y poder diseñar, programar y testear un software de exploración multimodal de datos de las ciencias del espacio. El presente trabajo se basa en la hipótesis de que ``mediante la presentación multimodal de datos astronómicos y astrofísicos se podría mejorar las técnicas actuales de despliego, promoviendo y facilitando la inclusión en el campo de la investigación''. Mediante esta investigación se estaría dando respuesta a los científicos que expresan la necesidad de nuevas formas de exploración de datos que permitan análisis de datos que no tengan una manipulación previa \citep{wandatesis2013}; y también a la necesidad de generar herramientas y prácticas que permitan la inclusión de personas con discapacidad en los ámbitos académicos y laborales.

La realidad actual de las ciencias espaciales es que la nueva generación de telescopios en tierra y en el espacio utilizan técnicas experimentales avanzadas para la captura de datos astrofísicos (energía electromagnética y partículas), con precisión y resolución temporal mejoradas. Sin embargo, aún se encuentran con limitaciones en el análisis de datos, algunas de ellas son:
\begin{enumerate}
    \item \textit{La ausencia de técnicas eficientes con bases adaptativas para detallar y analizar datos no lineales y no estacionarios}: la definición de la base es dependiente de los datos, suponiendo una base definida a posteriori, esto implica un enfoque muy diferente al análisis de datos matemáticos regulares \citep{bendat1993}. Usando la sonorización y la percepción humana, la base podría ser definida a posteriori.
    \item \textit{La limitación en la utilización de la presentación visual de los datos}: estos generalmente contienen mucha más información que la que puede ser efectivamente desplegada usando las tecnologías disponibles actualmente.  
    \item \textit{La habilidad humana para interpretar los datos del espacio extendido, limitada por la visualización y la perceptualización de los datos}: actualmente se trabajan en esta limitación filtrando (priorizando) los datos para desplegar sólo la información que se cree es importante para el problema que se estudia, esto lleva a hacer algunas suposiciones sobre el resultado, se estima que algunos descubrimientos pueden haberse perdido.
    \item \textit{Los métodos estándar de análisis de datos también hacen a la astronomía inaccesible} para personas física o sensorialmente discapacitadas (ciegos, orientados de forma auditiva, o quienes sufren desórdenes cognitivos). Esta investigación persigue reducir esta brecha.
\end{enumerate}

En búsqueda de mejorar las limitaciones expuestas anteriormente y salvar la falta de inclusión encontrada, se proponen los siguientes objetivos generales:
\begin{itemize}
    \item Investigar sobre nuevas modalidades de acceso a los datos astronómicos y astrofísicos, promoviendo la inclusión en los espacios científicos y buscando mejorar la forma de despliegue actual.
    \item Producir herramientas y documentación orientada a mejorar el acceso a los datos promoviendo la inclusión.
\end{itemize}

Con el fin de lograr los objetivos generales planteados, se proponen los siguientes objetivos específicos:
\begin{itemize}
    \item Revisión bibliográfica sobre el tema y de los software existentes para sonorización de datos.
    \item Estudio de normativas vigentes para la realización de programas e interfaces accesibles, y producción de una herramienta basado en software libre (por ejemplo Python).
    \item Realización de un grupo focal integrado por personas con y sin discapacidad visual, para investigación sobre usabilidad y accesibilidad del programa desarrollado.
    \item Rediseño de la interfaz humano computadora a partir de la investigación previa; planteamiento de posibles mejoras e inclusión de funcionalidades al programa. 
    \item Recuperación de datos de bases de datos especificas (por ejemplo: SIMBAD, NASA, SDSS, ADSAbs) para las pruebas técnicas de la herramienta de despliegue multimodal y pruebas con usuarios.
    \item Publicación de los resultados y transferencia a la comunidad.
\end{itemize}

En base a los objetivos planteados y con el objetivo de describir de la mejor forma posible la investigación y desarrollo realizados durante esta tesis, se ha dividido el escrito en siete (7) capítulos. En primer lugar se describe la base y punto de partida de este trabajo, encontrando en el Capítulo \ref{cap:marco_teorico} información sobre la discapacidad, el diseño centrado en el usuario y el actual enfoque multisensorial en las ciencias del espacio. Complementando lo mencionado, el Capítulo \ref{cap:estado_del_arte} describe las herramientas de sonorización existentes, haciendo una distinción entre las que existían antes de 2017 y las que han sido desarrolladas a lo largo de estos años de forma paralela con el desarrollo propio de esta tesis.

Los siguientes cinco (5) capítulos se describen prácticamente de forma cronológica. El Capítulo \ref{cap:analisis_normativo} contiene el análisis normativo realizado al iniciar el trabajo donde se evaluaron las herramientas existentes en 2017 y su accesibilidad, también se realizó un estudio de accesibilidad a tres bases de datos astronómicas, decantando en un documento con recomendaciones de accesibilidad y el primer diseño de interfaz gráfica para el software sonoUno (descripto a lo largo de los últimos cuatro (4) capítulos). El Capítulo \ref{cap:sonouno_v1} describe el desarrollo de la primer versión de sonoUno, disponible para Windows, MacOS y Ubuntu.

Una vez que se logró la primer versión del software de sonorización, se realizó la primer prueba con usuarios de forma presencial en la Universidad de Southampton, Reino Unido. Dicho trabajo se describe en el Capítulo \ref{cap:fg_completo} junto con las pruebas realizadas a distancia con contactos de diferentes partes del mundo, para éstas últimas, las comunicaciones se realizaron por mail y a través de una encuentra en Google Form. Adicionalmente, al final del Capítulo \ref{cap:fg_completo} se presentan dos casos donde se utiliza el programa sonoUno para sonorización de datos astronómicos.

Durante el desarrollo de esta tesis, además de trabajar sobre la interfaz gráfica y su accesibilidad, se desarrollaron nuevas sonorizaciones de datos de grandes facilidades astrofísicas y bases de datos. En el Capítulo \ref{cap:reinforce} se detallan los desarrollos sobre sonorización de partículas del Gran Colisionador de Hadrones, imágenes y datos de muongrafía. Además, se agregan ejemplos de aplicación del software a espectros de galaxia, estrellas variables y rayos cósmicos. En este mismo capítulo se describe la versión web de la herramienta y los primeros pasos para lograr una plataforma de sonorización de datos que unifique las diferentes versiones del programa.

Finalmente, el Capítulo \ref{cap:sonouno_vfinal} se dedicó a describir la página web con información dedicada al proyecto sonoUno, allí se encuentran también los manuales de instalación y de usuario, los accesos a la herramienta, una sección de noticias y una galería que muestra diferentes datos y sus sonorizaciones. Se incluye en el Capítulo \ref{cap:sonouno_vfinal} un apartado con el primer entrenamiento en sonorización realizado durante 2022 dentro del equipo de trabajo y un apartado que establece las bases para futuros desarrollos e investigaciones.

Desde 2017 que se inició con esta investigación se han ido realizando transferencias a la comunidad junto con publicaciones científicas que le fueron dando pautas al equipo de trabajo de que se estaba dirigiendo en la dirección correcta. Se ha participado de numerosos congresos presentando los avances (se incluyen las publicaciones en las secciones correspondientes), desde 2019 se participó en un proyecto de colaboración internacional (proyecto REINFORCE, descripto en el Capítulo \ref{cap:reinforce}) y se recibió invitación para participar del Audible Universe Workshop 1 y 2 (un encuentro que desde su primer edición en 2021 se ha realizado de forma anual convocando a especialistas en sonorización de diferentes áreas de estudio).

